Devil is in the Uniformity: Exploring Diverse Learners within Transformer for Image Restoration

Transformer-based approaches have gained significant attention in image restoration, where the core component, i.e, Multi-Head Attention (MHA), plays a crucial role in capturing diverse features and recovering high-quality results. In MHA, heads perform attention calculation independently from uniform split subspaces, and a redundancy issue is triggered to hinder the model from achieving satisfactory outputs. In this paper, we propose to improve MHA by exploring diverse learners and introducing various interactions between heads, which results in a Hierarchical multI-head atteNtion driven Transformer model, termed HINT, for image restoration. HINT contains two modules, i.e., the Hierarchical Multi-Head Attention (HMHA) and the Query-Key Cache Updating (QKCU) module, to address the redundancy problem that is rooted in vanilla MHA. Specifically, HMHA extracts diverse contextual features by employing heads to learn from subspaces of varying sizes and containing different information. Moreover, QKCU, comprising intra- and inter-layer schemes, further reduces the redundancy problem by facilitating enhanced interactions between attention heads within and across layers. Extensive experiments are conducted on 12 benchmarks across 5 image restoration tasks, including low-light enhancement, dehazing, desnowing, denoising, and deraining, to demonstrate the superiority of HINT. The source code is available in the supplementary materials.

==> sec/0_abstract.tex <==
\begin{abstract}
% Transformer-based approaches have gained significant attention in image restoration, owing to their capability of modeling long-range dependencies and promising performance in addressing various degradations. 
%
% While diverse attention mechanisms have been proposed to enhance feature representation learning, few touch the core component of this mechanism, i.e., Multi-head Attention (MHA). 
Transformer-based approaches have gained significant attention in image restoration, where the core component, i.e, Multi-Head Attention (MHA), plays a crucial role in capturing diverse features and recovering high-quality results. 
%
In MHA, heads perform attention calculation independently from uniform split subspaces, and a redundancy issue is triggered to hinder the model from achieving satisfactory outputs. 
%
% In this paper, we propose to address the redundant issue inherent in the vanilla MHA, and results in a \textbf{H}ierarchical mult\textbf{I}-head atte\textbf{N}tion driven \textbf{T}ransformer model, termed HINT, for image restoration. 
In this paper, we propose to improve MHA by exploring diverse learners and introducing various interactions between heads, which results in a \textbf{H}ierarchical mult\textbf{I}-head atte\textbf{N}tion driven \textbf{T}ransformer model, termed HINT, for image restoration. 
%
% The success of HINT lies in the combination of two key ingredients, i.e., the Hierarchical Multi-Head Attention (HMHA) module and the Query-Key Cache Updating (QKCU) mechanism. 
%
HINT contains two modules, i.e., the Hierarchical Multi-Head Attention (HMHA) and the Query-Key Cache Updating (QKCU) module, to address the redundancy problem that is rooted in vanilla MHA. 
%
Specifically, HMHA extracts diverse contextual features by employing heads to learn from subspaces of varying sizes and containing different information. 
%
Moreover, QKCU, comprising intra- and inter-layer schemes, further reduces the redundancy problem by facilitating enhanced interactions between attention heads within and across layers. 
%
Extensive experiments are conducted on \textbf{12} benchmarks across \textbf{5} image restoration tasks, including low-light enhancement, dehazing, desnowing, denoising, and deraining, to demonstrate the superiority of HINT. 
%
\textbf{The source code is available in the \textcolor{magenta}{supplementary materials}}.
\end{abstract}

==> sec/1_intro__old.tex <==
\section{Introduction}
\label{sec:intro}

The goal of image restoration is to recover clear images from their degraded versions. 
%
Given the fact that the quality of inputs can largely impact the performance of downstream high-level applications~\cite{ChenJPSWY24,DuanBXQHT24,0001HJH24}, image restoration is essential.
%
Over the past few decades, significant progress has been made by learning-based methods~\cite{yuke_pami22_car_blur_noise,chen2021pre,nips21_luo_sr} over hand-craft schemes~\cite{cho2009fast,fergus2006removing}. 
%
% In particular, CNN-based methods~\cite{cvpr2021cho, MIRNetv2} have limitations in modeling global relationships due to the restricted receptive field. 
%
% Recently, more advances have been achieved by Transformer-based pipelines~\cite{zamir2022restormer,iccv2021_swinIR} due to their capability to capture long-range dependencies. 
In particular, advances have been achieved by Transformer-based pipelines~\cite{zamir2022restormer,iccv2021_swinIR} due to their capability to capture long-range dependencies. 

\begin{figure}[tp!]
\centering
\includegraphics[width=.95\linewidth,height=6.5cm]{./Figures/manuscript/motivation_crop.pdf}
\vspace{-2mm}
\caption{ 
Illustration of the vanilla Multi-Head Attention (MHA) mechanism, which is widely adopted in existing methods~\cite{zamir2022restormer,iccv2021_swinIR,retinexformer}. 
%
The standard MHA assigns $h$ heads with subspaces of the same dimension, and each head performs attention calculation independently. 
%
As a result, these heads intend to focus on the same regions (red boxes) and neglect the restoration of some degraded areas (yellow boxes), leading to an unsatisfactory output. 
}
\label{pic:motivation}
\vspace{-4mm}
\end{figure}
%
% To achieve efficient Transformer-based models for restoring high-quality outputs, emerging strategies~\cite{zhou2024AST,zamir2022restormer,liu2022tuformer} have been developed to improve MHA mechanism. 
% %
% % Emerging strategies~\cite{iccv2021_swinIR,zamir2022restormer,chen2021pre} have been developed to address the intense computation load issues associated with the vanilla self-attention~\cite{vaswani2017attention,iclr2021_vit} mechanism within the Transformer architecture. 
% %
% Yet, few of these approaches have focused on improving the core component of this mechanism, i.e., multi-head attention (MHA), which is responsible for extracting diverse contextual features from different subspaces. 
% %
% Indeed, the standard MHA mechanism is proven to be redundant, where specialized heads perform the majority of the work~\cite{acl_voita2019analyzing}. 
% %
% This insight has been widely validated in the context of NLP~\cite{wang2022improved,nguyen2022improving,MGK_icml22}, and has inspired new directions in computer vision~\cite{xiao2024improving}. 

Multi-Head Attention (MHA) is a core component in Transformer architecture, which is responsible for capturing diverse representative features by employing multiple heads to attend to information from different subspaces. 
%
Each head performs attention calculations in parallel and independently of the others. 
%
Such a simple design is empirically successful, while it causes the redundancy issue~\cite{acl_voita2019analyzing,nguyen2022improving,MGK_icml22} as the heads, which are assigned with subspaces of the same dimension and lack of interactions, intend to focus on the same region, as shown in Figure~\ref{pic:motivation}. 
%
To improve the MHA mechanism, previous works attempt to enhance the interaction or collaboration between heads~\cite{ahmed2017weighted,acl_li2019information,emnlp_2022_mixture}. 
%
In a nutshell, they introduce sophisticated fusion modules to replace the simple concatenate-and-project paradigm in MHA. 
%
Unfortunately, these heads still operate independently and the underlying information exchange between tokens is not conducted. 
%
As a result, limited benefits of enhancing the representation ability can be earned in this way~\cite{xiao2024improving}. 
%
% Unfortunately, limited benefits in terms of expressive power can be earned in this way~\cite{xiao2024improving}, as the heads still operate independently, and the underlying information exchange between tokens is not considered. 
%
An alternative approach is to pay attention to the lowest level in the computation graph of the MHA~\cite{cordonnier2020multi,liu2022tuformer}, specifically by modulating the query, key, and value projections within each head. 
%
Operating directly on head projections does alter the information flow, while it incurs unfordable computation burden at the same time~\cite{xiao2024improving}.
% Operating directly on head projections does alter the information flow, while it lacks the adaptability to inputs due to its static nature~\cite{xiao2024improving}. 
%
More recently, a third solution has emerged, which involves modulating the attention score~\cite{shazeer2020talking,wang2022improved,nguyen2022improving}. 
%
In this way, minimal computation cost brings fundamental improvement in enhancing the representation ability of the model. 
%
Existing restoration models~\cite{DRSformer,zhou2024AST} adopt this paradigm to achieve better performance, however, they perform either the Top-K operation or new activation function on the already computed attention scores, lacking adaptability to inputs. 
%
% The full potential of modulating attention scores remains unrealized.

In this paper, we follow the basic idea of exploring efficient MHA and employ it to the problem of image restoration. 
%
We propose {HINT}, a \textbf{H}ierarchical multi-head atte\textbf{N}tion driven \textbf{T}ransformer model to remove undesired degradations from images. 
%
HINT follows the scheme to modulate the attention scores but makes it dynamic. 
% , and, more importantly, mitigate the redundant issue that is rooted in the vanilla MHA. 
%
As mentioned above, standard MHA~\cite{zamir2022restormer,iccv2021_swinIR} assigns each head with subspaces sharing the same dimension, which hampers the ability of each head to learn distinctive features and leads to redundancy as a result. 
%
In contrast, we propose to learn hierarchical multi-head attention (HMHA) that extracts diverse contextual information from heads using different dimensional subspaces. 
%
Additionally, we develop a Query-Key Cache Updating (QKCU) mechanism, comprising both intra- and inter-layer schemes, to enhance interaction among heads and boost performance. 
%
% Unlike existing restoration methods to implement modulation of attention scores in a static projection way~\cite{zhou2024AST,DRSformer}, we make the modulation dynamic, achieving better model expressiveness.

Overall, we summarize the contributions of this work:
%
\begin{itemize}
  \item  
  We present HINT, a \textbf{H}ierarchical multi-head atte\textbf{N}tion driven \textbf{T}ransformer model for image restoration. 
  %
  HINT demonstrates the effectiveness of learning hierarchical representations in Multi-Head Attention (MHA) and enhancing interactions via inter- and intra-layer ways for the problem of removing undesired degradations.
  \item HINT introduces the Hierarchical Multi-Head Attention (HMHA) module, which alleviates the redundancy issue in standard MHA by enabling the model to learn distinctive contextual features from different subspaces.
  %
  Additionally, HINT incorporates the Query-Key Cache Updating (QKCU) mechanism, combining intra- and inter-layer schemes to enhance interaction among heads. 
  \item Extensive qualitative and quantitative evaluations are conducted on \textbf{9} benchmarks for \textbf{3} typical image restoration tasks: dehazing, desnowing, and low-light enhancement, where HINT performs favorably against the state-of-the-art algorithms as well as strong baselines in terms of restored image quality.
  \end{itemize}



% \newpage

==> sec/6_supply.tex <==
% \clearpage
% \setcounter{page}{1}
% \maketitlesupplementary


This supplementary material provides additional details that could not be included in the main manuscript due to space constraints. 
%
It is organized as follows:
\begin{itemize}
\item Section~\ref{sec:supply_results} presents extended results for image restoration tasks along with an in-depth analysis of the proposed method.
% \item Section~\ref{sec:Limitation_Future} discusses the limitations of HIT and suggests potential techniques for future exploration.
\item Section~\ref{sec:Additional_Visual_Comparisons} showcases additional visual comparisons.
\item Section~\ref{sec:appedix_dataset} provides details on the datasets and experimental settings for each image restoration task. 
\end{itemize} 

\section{Additional Experiment Results}
\label{sec:supply_results}

\subsection{Image deraining}
We compare HINT with state-of-the-art deraining approaches on the Rain100L~\cite{fan2019general} benchmark. 
%
As shown in Table~\ref{tab:rain100L_supply}, HINT achieves the highest scores in terms of PSNR and SSIM metrics.
%
Compared to methods~\cite{jiang2020multi,wei2019semi,yasarla2019uncertainty,zhang2018density} that are specially designed for rain removal, our HINT demonstrates superior deraining performance. 
%
When compared to the restoration pipelines, including the all-in-one algorithms~\cite{potlapalli2024promptir,NDR-Restore_tip24,cui2025adair,li2022all} and general approaches~\cite{zamir2022restormer,zhou2025seeing}, HINT maintains consistent advantages. 


\subsection{Image enhancement}
We evaluate HINT against state-of-the-art image enhancement methods in the manuscript, following the widely adopted protocol~\cite{retinexformer} on the LOL-v2 benchmark~\cite{yang2021sparse}. 
%
Additionally, we note that some methods adopt an alternative evaluation setting, namely the `GT-mean' protocol, which the mean of the ground truth is used to obtain better results. 
%
As shown in Table~\ref{tab:enhancement_lolv2_gtmean}, HINT achieve competitive results on the LOL-v2-real subset and outperforms all methods on the LOL-v2-syn subset. 
%
Compared to the recent efficient network CIDNet~\cite{yan2024you} that specially designed for image enhancement, HINT obtains a significant 1.19 dB gain on PSNR, further demonstrating its effectiveness.


%Table rain
\begin{table}\footnotesize
\caption{Quantitative results on Rain100L~\cite{fan2019general} benchmark for rain-streak removal. }
\vspace{-2mm}
\centering
\footnotesize
% \scalebox{.716}
\setlength{\tabcolsep}{.305mm}
{
\begin{tabular}{ccccccccccccccc}
\toprule[0.8pt]
\multicolumn{1}{l}{\multirow{2}{*}{Method}} & \multicolumn{1}{c}{DIDMDN}   & \multicolumn{1}{c}{UMR} 
& \multicolumn{1}{c}{SIRR} &\multicolumn{1}{c}{MSPFN}
&\multicolumn{1}{c}{LPNet}&\multicolumn{1}{c}{AirNet}\\ 
\multicolumn{1}{l}{} & \multicolumn{1}{c}{{\scriptsize CVPR'18}}   & \multicolumn{1}{c}{{\scriptsize CVPR'19}} 
& \multicolumn{1}{c}{{\scriptsize CVPR'19}} &\multicolumn{1}{c}{{\scriptsize CVPR'20}}
&\multicolumn{1}{c}{{\scriptsize CVPR'19}}&\multicolumn{1}{c}{{\scriptsize CVPR’22}}\\ 
\multicolumn{1}{l}{{}} & \multicolumn{1}{c}{\cite{zhang2018density}}   & \multicolumn{1}{c}{\cite{yasarla2019uncertainty}} 
& \multicolumn{1}{c}{\cite{wei2019semi}} &\multicolumn{1}{c}{\cite{jiang2020multi}}
&\multicolumn{1}{c}{\cite{gao2019dynamic}}&\multicolumn{1}{c}{\cite{li2022all}}\\ 
\hline
\multicolumn{1}{l}{{PSNR}} & \multicolumn{1}{c}{23.79}   & \multicolumn{1}{c}{32.39} 
& \multicolumn{1}{c}{32.37} &\multicolumn{1}{c}{33.50}
&\multicolumn{1}{c}{33.61}&\multicolumn{1}{c}{34.90} 
\\
\multicolumn{1}{l}{{SSIM}} & \multicolumn{1}{c}{0.773}   & \multicolumn{1}{c}{0.921} 
& \multicolumn{1}{c}{0.926} &\multicolumn{1}{c}{0.948}
&\multicolumn{1}{c}{0.958}&\multicolumn{1}{c}{0.977} 
\\
\midrule[0.8pt]
\multicolumn{1}{l}{\multirow{2}{*}{Method}} & \multicolumn{1}{c}{Restormer}   & \multicolumn{1}{c}{PromptIR} 
& \multicolumn{1}{c}{NDR-Restore} &\multicolumn{1}{c}{AdaIR}
&\multicolumn{1}{c}{FPro}&\multicolumn{1}{c}{HINT}\\ 
\multicolumn{1}{l}{} & \multicolumn{1}{c}{{\scriptsize CVPR’22}}   & \multicolumn{1}{c}{{\scriptsize NeurIPS’23}} 
& \multicolumn{1}{c}{{\scriptsize TIP’24}} &\multicolumn{1}{c}{{\scriptsize ICLR’25}}
&\multicolumn{1}{c}{{\scriptsize ECCV'24}}&\multicolumn{1}{c}{-}\\ 
\multicolumn{1}{l}{{}} & \multicolumn{1}{c}{\cite{zamir2022restormer}}   & \multicolumn{1}{c}{\cite{potlapalli2024promptir}} 
& \multicolumn{1}{c}{\cite{NDR-Restore_tip24}} &\multicolumn{1}{c}{\cite{cui2025adair}}
&\multicolumn{1}{c}{\cite{zhou2025seeing}}&\multicolumn{1}{c}{(Ours)}\\ 
\hline
\multicolumn{1}{l}{{PSNR}} & \multicolumn{1}{c}{36.74}   & \multicolumn{1}{c}{37.04} 
& \multicolumn{1}{c}{38.33} &\multicolumn{1}{c}{38.90}
&\multicolumn{1}{c}{39.20}&\multicolumn{1}{c}{\textbf{40.04}} 
\\
\multicolumn{1}{l}{{SSIM}} & \multicolumn{1}{c}{0.978}   & \multicolumn{1}{c}{0.979} 
& \multicolumn{1}{c}{0.984} &\multicolumn{1}{c}{\underline{0.985}}
&\multicolumn{1}{c}{\underline{0.985}}&\multicolumn{1}{c}{\textbf{0.986}} 
\\
\bottomrule[0.8pt]
\vspace{-4mm}
\end{tabular}}
\label{tab:rain100L_supply}
\end{table}


\begin{table}[!t]
\caption{Quantitative comparisons on LOL-v2~\cite{yang2021sparse} with `GT-mean' protocol for low-light enhancement. 
}
\vspace{-2mm}
\centering
\footnotesize
% \scalebox{1.}
\setlength{\tabcolsep}{.5mm}
{
\begin{tabular}{cccccccccc}
\toprule
% \multicolumn{2}{l}{\textbf{}}   & \multicolumn{4}{l}{{SMID}
% }\\ 
% \cline{3-6} 
\multicolumn{2}{l|}{{Method}}  & \multicolumn{2}{c|}{LOL-v2-real}  & \multicolumn{2}{c|}{LOL-v2-syn}& \multicolumn{2}{c}{Average}\\  
\multicolumn{2}{l|}{}  & \multicolumn{1}{c}{{PSNR}}  & \multicolumn{1}{c|}{{SSIM}}& \multicolumn{1}{c}{{PSNR}}  & \multicolumn{1}{c|}{{SSIM}}& \multicolumn{1}{c}{{PSNR}}  & \multicolumn{1}{c}{{SSIM}}\\  
\midrule
\multicolumn{2}{l|}{LLFlow~\cite{wang2022low}{\scriptsize(AAAI'22)}}  & \multicolumn{1}{c}{{26.53}} & \multicolumn{1}{c|}{{0.892}}& \multicolumn{1}{c}{{26.23}} & \multicolumn{1}{c|}{{0.943}}& \multicolumn{1}{c}{{26.38}} & \multicolumn{1}{c}{{0.918}}\\

\multicolumn{2}{l|}{Retinexformer~\cite{retinexformer}{\scriptsize(ICCV'23)}}  & \multicolumn{1}{c}{{27.71}} & \multicolumn{1}{c|}{{0.856}}& \multicolumn{1}{c}{{29.04}} & \multicolumn{1}{c|}{{0.939}}& \multicolumn{1}{c}{{28.38}} & \multicolumn{1}{c}{{0.898}}\\

\multicolumn{2}{l|}{GLARE~\cite{zhou2024glare}{\scriptsize(ECCV'24)}}  & \multicolumn{1}{c}{\textbf{28.98}} & \multicolumn{1}{c|}{\textbf{0.905}}& \multicolumn{1}{c}{\underline{29.84}} & \multicolumn{1}{c|}{\underline{0.958}}& \multicolumn{1}{c}{\underline{29.41}} & \multicolumn{1}{c}{\textbf{0.932}}\\

% \multicolumn{2}{l|}{ECMamba~\cite{dong2025ecmamba}{\scriptsize(NeurIPS'24)}}  & \multicolumn{1}{c}{\textbf{29.24}} & \multicolumn{1}{c|}{\textbf{0.908}}& \multicolumn{1}{c}{\underline{29.94}} & \multicolumn{1}{c|}{\textbf{0.959}}& \multicolumn{1}{c}{\underline{29.59}} & \multicolumn{1}{c}{\textbf{0.934}}\\
\multicolumn{2}{l|}{CIDNet~\cite{yan2024you}{\scriptsize(CVPR'25)}}  & \multicolumn{1}{c}{28.14} & \multicolumn{1}{c|}{0.892}& \multicolumn{1}{c}{29.37} & \multicolumn{1}{c|}{0.950}& \multicolumn{1}{c}{28.76} & \multicolumn{1}{c}{\underline{0.921}}\\

\hline
\multicolumn{2}{l|}{HINT (Ours)} & \multicolumn{1}{c}{\underline{28.82}} & \multicolumn{1}{c|}{\underline{0.904}} & \multicolumn{1}{c}{\textbf{31.07}}  & \multicolumn{1}{c|}{\textbf{0.959}}& \multicolumn{1}{c}{\textbf{29.95}} & \multicolumn{1}{c}{\textbf{0.932}}\\ 
\bottomrule
\vspace{-4mm}
\end{tabular}}
\label{tab:enhancement_lolv2_gtmean}
\end{table}

\subsection{Image denosing}
For image denoising, we perform experiments on BSD68 \cite{martin2001database} and Urban100 \cite{huang2015single}. 
%
As shown in Table~\ref{tab:desnoising_supply}, HINT performs favorably against state-of-the-art denoising methods. 
%
Compared to the strong competitor Restormer~\cite{zamir2022restormer}, HINT achieves an average gain of 0.2 dB in PSNR. 
%
Our HINT surpasses previous methods in all-in-one paradigms~\cite{li2022all,potlapalli2024promptir,NDR-Restore_tip24}, delivering at least 0.12 dB performance gain.

\begin{table*}[!tp]
\caption{Quantitative comparisons on BSD68 \cite{martin2001database} and Urban100 \cite{huang2015single} for denosing. 
}
% \vspace{-2mm}
\centering
\footnotesize
% \scalebox{1.}
% \setlength{\tabcolsep}{1.5mm}
{
\begin{tabular}{cccccccc}
\toprule
% \multicolumn{2}{l}{\textbf{}}   & \multicolumn{4}{l}{{SMID}
% }\\ 
% \cline{3-6} 
\multicolumn{1}{l|}{{Method}}  & \multicolumn{3}{c|}{BSD68 \cite{martin2001database}}  & \multicolumn{3}{c|}{Urban100 \cite{huang2015single}} & \multicolumn{1}{c}{Average}\\  
\multicolumn{1}{l|}{}  & \multicolumn{1}{c}{{$\sigma$=15}}  & \multicolumn{1}{c}{{$\sigma$=25}}& \multicolumn{1}{c|}{{$\sigma$=50}}  & \multicolumn{1}{c}{{$\sigma$=15}}  & \multicolumn{1}{c}{{$\sigma$=25}}& \multicolumn{1}{c|}{{$\sigma$=50}} & \multicolumn{1}{c}{}  \\  
\midrule
\multicolumn{1}{l|}{CBM3D \cite{dabov2007color} ({\scriptsize ICIP'07})}   & \multicolumn{1}{c}{33.50/0.922}  & \multicolumn{1}{c}{30.69/0.868}& \multicolumn{1}{c|}{27.36/0.763}  & \multicolumn{1}{c}{33.93/0.941}  & \multicolumn{1}{c}{31.36/0.909}& \multicolumn{1}{c|}{27.93/0.840} & \multicolumn{1}{c}{30.80/0.874}  \\  
\multicolumn{1}{l|}{DnCNN \cite{zhang2017tip} ({\scriptsize TIP'17})}  & \multicolumn{1}{c}{33.89/0.930}  & \multicolumn{1}{c}{31.23/0.883}& \multicolumn{1}{c|}{27.92/0.789}  & \multicolumn{1}{c}{32.98/0.931}  & \multicolumn{1}{c}{30.81/0.902}& \multicolumn{1}{c|}{27.59/0.833} & \multicolumn{1}{c}{30.74/0.878}  \\  
\multicolumn{1}{l|}{IRCNN \cite{zhang2017learning} ({\scriptsize CVPR'17})}  & \multicolumn{1}{c}{33.87/0.929}  & \multicolumn{1}{c}{31.18/0.882}& \multicolumn{1}{c|}{27.88/0.790}  & \multicolumn{1}{c}{27.59/0.833}  & \multicolumn{1}{c}{31.20/0.909}& \multicolumn{1}{c|}{27.70/0.840} & \multicolumn{1}{c}{29.90/0.864}  \\  
\multicolumn{1}{l|}{FFDNet \cite{tip2018ffdnet} ({\scriptsize TIP'18})}  & \multicolumn{1}{c}{33.87/0.929}  & \multicolumn{1}{c}{31.21/0.882}& \multicolumn{1}{c|}{27.96/0.789}  & \multicolumn{1}{c}{33.83/0.942}  & \multicolumn{1}{c}{31.40/0.912}& \multicolumn{1}{c|}{28.05/0.848} & \multicolumn{1}{c}{31.05/0.884}  \\  
\multicolumn{1}{l|}{BRDNet \cite{tian2020image} ({\scriptsize Neural Networks'20})}  & \multicolumn{1}{c}{34.10/0.929}  & \multicolumn{1}{c}{31.43/0.885}& \multicolumn{1}{c|}{28.16/0.794}  & \multicolumn{1}{c}{34.42/0.946}  & \multicolumn{1}{c}{31.99/0.919}& \multicolumn{1}{c|}{28.56/0.858} & \multicolumn{1}{c}{31.44/0.889}  \\  
\multicolumn{1}{l|}{AirNet \cite{li2022all} ({\scriptsize CVPR'22})}  & \multicolumn{1}{c}{34.14/0.936}  & \multicolumn{1}{c}{31.48/0.893}& \multicolumn{1}{c|}{28.23/0.806}  & \multicolumn{1}{c}{34.40/0.949}  & \multicolumn{1}{c}{32.10/0.924}& \multicolumn{1}{c|}{28.88/0.871} & \multicolumn{1}{c}{31.54/0.897}  \\  
\multicolumn{1}{l|}{Restormer \cite{zamir2022restormer} ({\scriptsize CVPR'22})}  & \multicolumn{1}{c}{34.29/\underline{0.937}}  & \multicolumn{1}{c}{31.64/\underline{0.895}}& \multicolumn{1}{c|}{28.41/0.810}  & \multicolumn{1}{c}{34.67/\textbf{0.969}}  & \multicolumn{1}{c}{32.41/\underline{0.927}}& \multicolumn{1}{c|}{29.31/{0.878}} & \multicolumn{1}{c}{31.79/\textbf{0.903}}  \\  
\multicolumn{1}{l|}{PromptIR \cite{potlapalli2024promptir} ({\scriptsize NeurIPS'23})}  & \multicolumn{1}{c}{\underline{34.34}/\textbf{0.938}}  & \multicolumn{1}{c}{\underline{31.71}/\textbf{0.897}}& \multicolumn{1}{c|}{\underline{28.49}/\textbf{0.813}}  & \multicolumn{1}{c}{34.77/\underline{0.952}}  & \multicolumn{1}{c}{\underline{32.49}/\textbf{0.929}}& \multicolumn{1}{c|}{\underline{29.39}/\underline{0.881}} & \multicolumn{1}{c}{\underline{31.87}/\underline{0.902}}  \\ 
\multicolumn{1}{l|}{NDR-Restore \cite{NDR-Restore_tip24} ({\scriptsize TIP'24})}  & \multicolumn{1}{c}{34.30/0.936}  & \multicolumn{1}{c}{31.65/0.892}& \multicolumn{1}{c|}{28.38/0.807}  & \multicolumn{1}{c}{\underline{34.80}/0.950}  & \multicolumn{1}{c}{32.48/0.926}& \multicolumn{1}{c|}{29.31/0.877} & \multicolumn{1}{c}{31.82/0.898}  \\
% \multicolumn{1}{l|}{AdaIR \cite{cui2025adair} ({\scriptsize ICLR'25})}  & \multicolumn{1}{c}{34.36/0.938}  & \multicolumn{1}{c}{31.72/0.897}& \multicolumn{1}{c|}{28.49/0.813}  & \multicolumn{1}{c}{34.96/0.953}  & \multicolumn{1}{c}{32.74/0.931}& \multicolumn{1}{c|}{29.70/0.885} & \multicolumn{1}{c}{32.00/0.903}  \\
\hline
\multicolumn{1}{l|}{HINT (Ours)}  & \multicolumn{1}{c}{\textbf{34.36}/0.935}  & \multicolumn{1}{c}{\textbf{31.74}/0.894}& \multicolumn{1}{c|}{\textbf{28.55}/\underline{0.812}}  & \multicolumn{1}{c}{ \textbf{34.91}/0.951}  & \multicolumn{1}{c}{ \textbf{32.70}/\textbf{0.929}}& \multicolumn{1}{c|}{\textbf{29.70}/\textbf{0.884}} & \multicolumn{1}{c}{\textbf{31.99}/0.901}  \\
%180000/300000

\bottomrule
\vspace{-4mm}
\end{tabular}}
\label{tab:desnoising_supply}
\end{table*}

\subsection{Comparison to Image Restoration Baselines}
% \label{sec:appedix_baselineComparison}
We compare HINT with the general restoration baselines, including Uformer~\cite{liu2022tuformer} and Restormer~\cite{zamir2022restormer}, to demonstrate its effectiveness. 
%
As illustrated in Fig.~\ref{pic:PSNRcomp}, HINT consistently outperforms these methods across all tasks, achieving the highest scores on key benchmarks, such as haze removal on SOTS~\cite{li2018benchmarking}, snow removal on Snow100K~\cite{liu2018desnownet}, and low-light enhancement on LOL-v2~\cite{yang2021sparse}.

\begin{figure}[t]
% \scriptsize
\centering
\begin{tabular}{c}
\includegraphics[width=0.45\textwidth]{Figures/supply/radar_HINT.pdf}
\end{tabular}
\vspace{-2mm}
\caption{PSNR comparison with baseline models across 3 tasks. 
% Best viewed in color.
}
\label{pic:PSNRcomp}
\vspace{-4mm}
\end{figure}


\begin{figure*}[!t]
% \scriptsize
\footnotesize
\centering
\begin{tabular}{ccc}
% % one row
% \hspace{-0.42cm}
\begin{adjustbox}{valign=t}
\begin{tabular}{cccc}
\hspace{-.42cm}
\adjustbox{valign=t}{\includegraphics[width=0.24\textwidth]{Figures/patches/snowyInput.jpg} }\hspace{-4mm} &
% \hspace{-.8032cm}
\adjustbox{valign=t}{\includegraphics[width=0.24\textwidth]{Figures/patches/snowyInput_detect.png} }\hspace{-4mm} &
% \hspace{-.8032cm}
\adjustbox{valign=t}{\includegraphics[width=0.24\textwidth]{Figures/patches/snowyRestore.png} }\hspace{-4mm} &
% \hspace{-.8032cm}
\adjustbox{valign=t}{\includegraphics[width=0.24\textwidth]{Figures/patches/snowyRestore_detect.png} }\hspace{-4mm} 
\\
\hspace{-.42cm}
(a) Snowy Input \hspace{-4mm} &
(b) Detection result on (a) \hspace{-4mm} 
&
(c) Restored by HINT \hspace{-4mm} 
&
(d) Detection result on (c)  \hspace{-4mm} 
\\
\hspace{-.42cm}
\adjustbox{valign=t}{\includegraphics[width=0.24\textwidth]{Figures/patches/snowyInput2.jpg}} \hspace{-4mm} &
% \hspace{-.8032cm}
\adjustbox{valign=t}{\includegraphics[width=0.24\textwidth]{Figures/patches/snowyInput_seg.png}} \hspace{-4mm} &
% \hspace{-.8032cm}
\adjustbox{valign=t}{\includegraphics[width=0.24\textwidth]{Figures/patches/snowyRestore2.png}} \hspace{-4mm} &
% \hspace{-.8032cm}
\adjustbox{valign=t}{\includegraphics[width=0.24\textwidth]{Figures/patches/snowyRestore_seg.png}} \hspace{-4mm} 
\\
\hspace{-.42cm}
(e) Snowy Input  \hspace{-4mm} & 
(f) Segmentation result on (e)  \hspace{-4mm} &
(g) Restored by HINT \hspace{-4mm} & 
(h) Segmentation result on (g)  \hspace{-4mm} 
\end{tabular}
\end{adjustbox}
\end{tabular}
\vspace{-2mm}
\caption{The results of high-level computer vision tasks from the degraded and restored images. 
%
The restored image produced by HINT could boost the performance of downstream tasks~(i.e., Object Detection and Semantic Segmentation), where the false negative examples (e.g., the cows and the sky in the restored image) can be successfully detected or segmented.}
\label{pic:downstream_highlevel_tasks}
\end{figure*}


\subsection{Application to High-level Vision Tasks}
% \label{sec:downstream_highlevel_tasks}
In the main paper, we demonstrated the application of HINT to low-light object detection.
%
Here, we further showcase how images restored by HINT can enhance the performance of downstream high-level vision tasks, such as object detection\footnote{Object detection results and confidence scores are obtained using the DETR-ResNet-50 model~\cite{carion2020end} via the Hugging Face API: \url{https://huggingface.co/facebook/detr-resnet-50}.} and semantic segmentation\footnote{Semantic segmentation results are provided by SAM (Segment Anything Model)~\cite{kirillov2023segment} via its online API: \url{https://segment-anything.com/}.}.
%
As shown in Fig.~\ref{pic:downstream_highlevel_tasks}, HINT enables the successful detection or segmentation of previously missed objects, e.g., the cows in the top row and the sky in the bottom row, which were false negatives in degraded conditions.
%
This comparison highlights the effectiveness of HINT, not only in enhancing visual quality, but also in boosting performance for downstream vision tasks.

%LLOD_detail
\begin{table}[t]\footnotesize
\caption{Low-light object detection results on ExDark~\cite{loh2019getting}.}
% \vspace{-2mm}
\centering
% \small
\footnotesize
% \scriptsize
% \scalebox{1.2}
\setlength{\tabcolsep}{2.25mm}
{
\begin{tabular}{cccc}
\toprule[0.8pt]
% \multicolumn{2}{l|}{\textbf{Task}} & \multicolumn{2}{c}{haze}& \multicolumn{2}{c}{rain streak}&\multicolumn{2}{c}{shadow} &\multicolumn{2}{c}{snow}&\multicolumn{2}{c}{moir{\'e}}&\multicolumn{2}{c}{raindrop}&\multicolumn{2}{|c}{Avg}\\ 
% \cline{3-6} 
\multicolumn{1}{l|}{Class} & \multicolumn{1}{c}{Input}  &\multicolumn{1}{c|}{HINT} &\multicolumn{1}{c}{$\Delta$}\\ 
\midrule[0.8pt]
\multicolumn{1}{l|}{Bicycle} &\multicolumn{1}{c}{58.6}&\multicolumn{1}{c|}{63.9}&\multicolumn{1}{c}{+5.3}\\
\multicolumn{1}{l|}{Boat} &\multicolumn{1}{c}{43.0}&\multicolumn{1}{c|}{52.2}&\multicolumn{1}{c}{+9.2}\\
\multicolumn{1}{l|}{Bottle} &\multicolumn{1}{c}{43.1}&\multicolumn{1}{c|}{50.0}&\multicolumn{1}{c}{+6.9}\\
\multicolumn{1}{l|}{Bus} &\multicolumn{1}{c}{72.3}&\multicolumn{1}{c|}{74.1}&\multicolumn{1}{c}{+1.8}\\
\multicolumn{1}{l|}{Car} &\multicolumn{1}{c}{54.2}&\multicolumn{1}{c|}{58.2}&\multicolumn{1}{c}{+4.0}\\
\multicolumn{1}{l|}{Cat} &\multicolumn{1}{c}{37.6}&\multicolumn{1}{c|}{48.8}&\multicolumn{1}{c}{+11.2}\\
\multicolumn{1}{l|}{Chair} &\multicolumn{1}{c}{36.3}&\multicolumn{1}{c|}{49.0}&\multicolumn{1}{c}{+12.7}\\
\multicolumn{1}{l|}{Cup} &\multicolumn{1}{c}{39.6}&\multicolumn{1}{c|}{47.4}&\multicolumn{1}{c}{+7.8}\\
\multicolumn{1}{l|}{Dog} &\multicolumn{1}{c}{49.0}&\multicolumn{1}{c|}{59.3}&\multicolumn{1}{c}{+10.3}\\
\multicolumn{1}{l|}{Motorbike} &\multicolumn{1}{c}{35.1}&\multicolumn{1}{c|}{38.9}&\multicolumn{1}{c}{+3.8}\\
\multicolumn{1}{l|}{People} &\multicolumn{1}{c}{41.3}&\multicolumn{1}{c|}{50.9}&\multicolumn{1}{c}{+9.6}\\
\multicolumn{1}{l|}{Table} &\multicolumn{1}{c}{30.6}&\multicolumn{1}{c|}{40.2}&\multicolumn{1}{c}{+9.6}\\
\hline
\multicolumn{1}{l|}{Mean} &\multicolumn{1}{c}{45.1}&\multicolumn{1}{c|}{52.7}&\multicolumn{1}{c}{+7.6}\\
\bottomrule[0.8pt]
\vspace{-4mm}
\end{tabular}}
\label{tab:exdark_quantitative_detail}
\end{table}

As described in the manuscript, we conduct low-light object detection experiments on the ExDark~\cite{loh2019getting} benchmark for quantitative comparison. 
%
Table~\ref{tab:exdark_quantitative_detail} presents detailed results across different object classes.
%
Overall, the enhanced results demonstrate consistent improvements across all categories, with performance gains reaching up to 12.7 (Chair).

\subsection{More Ablation Study} 
We further investigate the design choices in HINT from three perspectives: (1) dimensional ratio in HMHA as shown in Table~\ref{tab:aba_dimensionRatio_supply}, (2) similarity functions used in the reranking strategy as shown in Table~\ref{tab:supply_similarity}, and (3) sensitivity analysis of the hyper-parameter $\alpha$ in Equation~(9) of the manuscript, as illustrated in Figure~\ref{pic:PSNRcomp_alpha}. 
%


% \clearpage

%Aba HMHA
\begin{table}
\caption{Ablation study of dimension ratio in HMHA. 
}
% \vspace{-2.mm}
\centering
\footnotesize
% \scalebox{0.850350}
\setlength{\tabcolsep}{5.05mm}
{
\begin{tabular}{ccc}
\toprule[0.8pt]
\multicolumn{1}{c}{}%& \multicolumn{2}{c}{\textbf{Reshape}}
& \multicolumn{1}{c}{{dimensional ratio}}%& \multicolumn{2}{c}{\textbf{Conv}} 
& \multicolumn{1}{|c}{{PSNR}}
 \\ \midrule[0.8pt]

\multicolumn{1}{c}{(a)} &\multicolumn{1}{c}{[1,1,1,5]} &\multicolumn{1}{|c}{26.71}  \\
\multicolumn{1}{c}{(b)} &\multicolumn{1}{c}{[1,1,2,4]} &\multicolumn{1}{|c}{26.91}  \\
\multicolumn{1}{c}{(c)} &\multicolumn{1}{c}{[1,2,2,3]} &\multicolumn{1}{|c}{27.17}  \\
\multicolumn{1}{c}{(d)} &\multicolumn{1}{c}{[1,1,3,3]} &\multicolumn{1}{|c}{26.70}  \\
  
\bottomrule
\end{tabular}}\textbf{}

\label{tab:aba_dimensionRatio_supply}
% \vspace{-5.5mm}
% \vspace{-3mm}
\end{table}

%Aba HMHA
\begin{table}
\caption{Ablation study of similarity functions in HMHA. 
}
% \vspace{-2.mm}
\centering
\footnotesize
% \scalebox{0.850350}
\setlength{\tabcolsep}{5.05mm}
{
\begin{tabular}{ccc}
\toprule[0.8pt]
\multicolumn{1}{c}{}%& \multicolumn{2}{c}{\textbf{Reshape}}
& \multicolumn{1}{c}{{function}}%& \multicolumn{2}{c}{\textbf{Conv}} 
& \multicolumn{1}{|c}{{PSNR}}
 \\ \midrule[0.8pt]

\multicolumn{1}{c}{(a)} &\multicolumn{1}{c}{Cosine Similarity} &\multicolumn{1}{|c}{26.62}  \\
\multicolumn{1}{c}{(b)} &\multicolumn{1}{c}{Manhattan Distance} &\multicolumn{1}{|c}{26.59}  \\
\multicolumn{1}{c}{(c)} &\multicolumn{1}{c}{Pearson Correlation Coefficient} &\multicolumn{1}{|c}{27.17}  \\
\multicolumn{1}{c}{(d)} &\multicolumn{1}{c}{Dot Product} &\multicolumn{1}{|c}{27.01}  \\

  
\bottomrule
\end{tabular}}\textbf{}

\label{tab:supply_similarity}
% \vspace{-5.5mm}
% \vspace{-3mm}
\end{table}


% \clearpage
\begin{figure}[t]
% \scriptsize
\centering
\begin{tabular}{c}
\includegraphics[width=0.45\textwidth]{Figures/supply/chart_alpha.pdf}
\end{tabular}
\vspace{-2mm}
\caption{The hyper-parameter sensitivity. 
% Best viewed in color.
}
\label{pic:PSNRcomp_alpha}
\vspace{-4mm}
\end{figure}

\section{Additional Visual Comparisons}
\label{sec:Additional_Visual_Comparisons}
To further demonstrate the effectiveness of HINT, we provide more visual results of our HINT on image deraining (Figure~\ref{pic:vis_derain_supply_derain100L}), image dehazing (Figure~\ref{pic:vis_dehaze_supply_sots}), image enhancement (Figure~\ref{pic:vis_realworld_supply} and Figure~\ref{pic:enhancement_lolv2_supply}), image desnowing (Figure~\ref{pic:snow_supply}), image denoising (Figure~\ref{pic:vis_dehnoising_supply_BSD68}). 
%
These visual comparisons highlight the effect of HINT across diverse degradation scenarios.


\section{Detailed Experimental Settings}
\label{sec:appedix_dataset}
We summarize the datasets used for training and evaluation in Table~\ref{tab:tasks_summary}. Below, we provide detailed descriptions for each individual task.

\begin{table}
\caption{Summary of various image restoration tasks datasets.} %S, S+ and R represent that images are generated by algorithm, taken from simulated scenes and real-world scenes respectively.}
% \vspace{-3mm}
\centering
% \small
\footnotesize
\setlength{\tabcolsep}{1.5mm}
{
\begin{tabular}{ccccc}
\toprule[0.8pt]
\multicolumn{1}{c}{Tasks} & \multicolumn{1}{c}{Dataset} & \multicolumn{1}{c}{Train Samples}& \multicolumn{1}{c}{Test Samples}   & \multicolumn{1}{c}{Type} 
\\ 
% \cline{3-6} 
\midrule[0.8pt]

\multicolumn{1}{c}{\multirow{2}{*}{snow}}&\multicolumn{1}{c}{Snow100K~\cite{liu2018desnownet}} & \multicolumn{1}{c}{2500}& \multicolumn{1}{c}{2000}   & \multicolumn{1}{c}{{Syn}}
\\ 
\multicolumn{1}{c}{}&\multicolumn{1}{c}{Realistic~\cite{liu2018desnownet}} & \multicolumn{1}{c}{0}& \multicolumn{1}{c}{1329}   & \multicolumn{1}{c}{Real}
\\
\hline
 \multicolumn{1}{c}{haze} &\multicolumn{1}{c}{SOTS~\cite{li2018benchmarking}} & \multicolumn{1}{c}{72,135 }& \multicolumn{1}{c}{500}& \multicolumn{1}{c}{Syn} 
\\ 
\hline
\multicolumn{1}{c}{\multirow{6}{*}{low-light}}&\multicolumn{1}{c}{LOL-v2-real~\cite{yang2021sparse}} & \multicolumn{1}{c}{689}& \multicolumn{1}{c}{100}& \multicolumn{1}{c}{Real} 
\\ 
\multicolumn{1}{c}{}&\multicolumn{1}{c}{LOL-v2-syn~\cite{yang2021sparse}} & \multicolumn{1}{c}{900}& \multicolumn{1}{c}{100}& \multicolumn{1}{c}{Syn} 
\\ 
\multicolumn{1}{c}{}&\multicolumn{1}{c}{DICM~\cite{lee2013contrast}} & \multicolumn{1}{c}{0}& \multicolumn{1}{c}{69}& \multicolumn{1}{c}{Real} 
\\ 
\multicolumn{1}{c}{}&\multicolumn{1}{c}{MEF~\cite{ma2015perceptual}} & \multicolumn{1}{c}{0}& \multicolumn{1}{c}{17}& \multicolumn{1}{c}{Real} 
\\ 
\multicolumn{1}{c}{}&\multicolumn{1}{c}{NPE~\cite{wang2013naturalness}} & \multicolumn{1}{c}{0}& \multicolumn{1}{c}{8}& \multicolumn{1}{c}{Real} 
\\ 
\multicolumn{1}{c}{}&\multicolumn{1}{c}{VV~\cite{vonikakis2018evaluation}} & \multicolumn{1}{c}{0}& \multicolumn{1}{c}{24}& \multicolumn{1}{c}{Real} 
\\ 
\hline
 \multicolumn{1}{c}{rain} &\multicolumn{1}{c}{Rain100L~\cite{fan2019general}} & \multicolumn{1}{c}{200}& \multicolumn{1}{c}{100}& \multicolumn{1}{c}{Syn} 
\\ 
\hline
\multicolumn{1}{c}{\multirow{4}{*}{noise}}&\multicolumn{1}{c}{BSD400~\cite{arbelaez2010contour}} & \multicolumn{1}{c}{400}& \multicolumn{1}{c}{-}& \multicolumn{1}{c}{Syn} \\
\multicolumn{1}{c}{}&\multicolumn{1}{c}{WED~\cite{ma2016waterloo}} & \multicolumn{1}{c}{4,744}& \multicolumn{1}{c}{-}& \multicolumn{1}{c}{Syn} 
\\ 
\multicolumn{1}{c}{}&\multicolumn{1}{c}{BSD68~\cite{martin2001database}} & \multicolumn{1}{c}{-}& \multicolumn{1}{c}{68}& \multicolumn{1}{c}{Syn} 
\\ 
\multicolumn{1}{c}{}&\multicolumn{1}{c}{Urban100~\cite{huang2015single}} & \multicolumn{1}{c}{-}& \multicolumn{1}{c}{100}& \multicolumn{1}{c}{Syn} 
\\ 
\bottomrule[0.8pt]
\end{tabular}}
\label{tab:tasks_summary}
% \vspace{-6mm}
\vspace{-3mm}
\end{table}

\noindent\textbf{Desnowing.} 
For image desnowing, we evaluate HINT on the Snow100K \cite{liu2018desnownet} benchmark. 
%
It contains 100,000 synthesized snowy images with corresponding snow-free images. 
%
It also includes 1,329 realistic snowy images. 
%
Following \cite{potlapalli2024promptir}, we conduct training and evaluation on the subset. 

\noindent\textbf{Dehazing.}
For image dehazing, we train HINT on the SOTS \cite{li2018benchmarking} benchmark, adhering to the setting in \cite{potlapalli2024promptir}.
%
It has 72,135 training samples and 500 test samples, all of which are synthesized data.
%
% Following \cite{potlapalli2024promptir}, we evaluate HINT on the full-size resolution images.

\noindent\textbf{Low-light Enhancement.}
For low-light image enhancement, we validate HINT on multiple datasets.
LOL-v2-syn \cite{yang2021sparse} is a synthetic dataset, which contains 900 training samples and 100 test samples.
LOL-v2-real \cite{yang2021sparse} is a real-world dataset with 689 training samples and 100 test samples.
%
We train HINT on each subset to perform validation, following \cite{retinexformer}. 
%
Meanwhile, we also utilize four real-world image datasets, including DICM \cite{lee2013contrast} with 69 test samples, MEF \cite{ma2015perceptual} with 17 test samples, NPE \cite{wang2013naturalness} with 8 test samples, and VV \cite{vonikakis2018evaluation} with 24 test samples.
%
HINT is pre-trained on the LOL-v2-syn subset and applied to the real-world images.

\noindent\textbf{Deraining.}
For image deraining, we validate HINT on the Rain100L \cite{fan2019general} benchmark.
%
Following the configuration in \cite{potlapalli2024promptir}, the training set contains 200 paired rainy-clean images, and the test set has 100 pairs for evaluation.
%

\noindent\textbf{Denoising.}
We perform experiments on the BSD400~\cite{arbelaez2010contour} and WED~\cite{ma2016waterloo} datasets with different noise levels for image denoising, following the experimental setting in Finally, \cite{potlapalli2024promptir}. 
%
The BSD400~\cite{arbelaez2010contour} dataset contains 400 training samples, while the WED~\cite{ma2016waterloo} dataset consists of 4,744 images. 
%
The model pre-trained on the two datasets is validated on the BSD68 \cite{martin2001database} and Urban100 \cite{huang2015single} benchmarks, which include 68 and 100 test images, respectively.

Finally, we provide a summary of the notations used in the main manuscript as well as the corresponding descriptions in Table~\ref{notation}. 




%Rain_Fig
\begin{figure}[htbp!]
% \footnotesize
\scriptsize
\centering
\begin{tabular}{ccc}
% % one row
\begin{adjustbox}{valign=t}
\begin{tabular}{ccccc}
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_rain_sup1/input_full.png}  &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_rain_sup1/gt_full.png}   &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_rain_sup1/airnet_full.png}  &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_rain_sup1/promptir_full.png}  &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_rain_sup1/hint_full.png}  
\\
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_rain_sup1/input_part.png}  &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_rain_sup1/gt_part.png}   &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_rain_sup1/airnet_part.png}  &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_rain_sup1/promptir_part.png}  &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_rain_sup1/hint_part.png}  
\\
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_rain_sup2/input_full.png}  &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_rain_sup2/gt_full.png}   &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_rain_sup2/airnet_full.png}  &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_rain_sup2/promptir_full.png}  &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_rain_sup2/hint_full.png}  
\\
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_rain_sup2/input_part.png}  &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_rain_sup2/gt_part.png}   &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_rain_sup2/airnet_part.png}  &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_rain_sup2/promptir_part.png}  &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_rain_sup2/hint_part.png}  
\\
\hspace{-3mm}(a) &
\hspace{-3mm}(b)   &   
\hspace{-3mm}(c)   &
\hspace{-3mm}(d)   &
\hspace{-3mm}(e) 
\\
\hspace{-3mm} Input &
\hspace{-3mm} Reference  &   
\hspace{-3mm} AirNet\cite{li2022all}  &
\hspace{-3mm} promptir\cite{potlapalli2024promptir}  &
\hspace{-3mm} HINT
\\
\end{tabular}
\end{adjustbox}
\end{tabular}
% \vspace{-2mm}
\caption{
Qualitative results on the Rain100L~\cite{fan2019general} benchmark for rain removal.
%
}
% \vspace{-4mm}
\label{pic:vis_derain_supply_derain100L}
\end{figure}

\newpage


%Haze_Fig
\begin{figure}[htbp!]
% \footnotesize
\scriptsize
\centering
\begin{tabular}{ccc}
% % one row
\begin{adjustbox}{valign=t}
\begin{tabular}{ccccc}
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_haze_supply/input_full.png}  &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_haze_supply/gt_full.png}   &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_haze_supply/airnet_full.png}  &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_haze_supply/ast_full.png}  &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_haze_supply/hint_full.png}  
\\
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_haze_supply/input_part.png}  &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_haze_supply/gt_part.png}   &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_haze_supply/airnet_part.png}  &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_haze_supply/ast_part.png}  &
\hspace{-3mm}\includegraphics[width=0.091\textwidth]{Figures/vis_haze_supply/hint_part.png}  
\\
\hspace{-3mm}(a)   &
\hspace{-3mm}(b)   &   
\hspace{-3mm}(c)   &
\hspace{-3mm}(d)   &
\hspace{-3mm}(e) 
\\
\hspace{-3mm} Input &
\hspace{-3mm} Reference  &   
\hspace{-3mm} AirNet\cite{li2022all}  &
\hspace{-3mm} AST\cite{zhou2024AST}  &
\hspace{-3mm} HINT
\\
\end{tabular}
\end{adjustbox}
\end{tabular}
\vspace{-2mm}
\caption{
Qualitative results on SOTS~\cite{li2018benchmarking} benchmark for haze removal.
%
}
\vspace{-4mm}
\label{pic:vis_dehaze_supply_sots}
\end{figure}




%realworld_fig
\begin{figure}[htbp!]
% \scriptsize
\footnotesize
\centering
\begin{tabular}{ccc}
\hspace{-0.42cm}
\begin{adjustbox}{valign=t}
\begin{tabular}{ccc}
\includegraphics[width=0.15\textwidth]{Figures/vis_realworld_sup/DICM_input.png} \hspace{-4mm} &
% \includegraphics[width=0.12\textwidth]{./Figures/vis_realworld/NPE_SNRNet.png} \hspace{-4mm} &
\includegraphics[width=0.15\textwidth]{Figures/vis_realworld_sup/DICM_SNR-Net.png} \hspace{-4mm} &
\includegraphics[width=0.15\textwidth]{Figures/vis_realworld_sup/DICM_Hint.png} \hspace{-4mm} 
\\
 Input \hspace{-4mm} &
% (b) SNRNet \hspace{-4mm} &
% 22.08 dB/LG-ShadowNet~\cite{liu2021lgshadow} \hspace{-4mm} &
 SNRNet~\cite{xu2022snr} \hspace{-4mm} &
 HINT \hspace{-4mm} 
\\
\includegraphics[width=0.15\textwidth,height=2cm]{Figures/vis_realworld_sup/MEF_input.png} \hspace{-4mm} &
% \includegraphics[width=0.12\textwidth]{./Figures/vis_realworld/DICM_SNRNet.png} \hspace{-4mm} &
\includegraphics[width=0.15\textwidth,height=2cm]{Figures/vis_realworld_sup/MEF_Sparse.png} \hspace{-4mm} &
\includegraphics[width=0.15\textwidth,height=2cm]{Figures/vis_realworld_sup/MEF_Hint.png} \hspace{-4mm} 
\\
 Input \hspace{-4mm} &
% (b) SNRNet \hspace{-4mm} &
% 22.08 dB/LG-ShadowNet~\cite{liu2021lgshadow} \hspace{-4mm} &
 Sparse~\cite{yang2021sparse} \hspace{-4mm} &
 HINT \hspace{-4mm} 
\\
\includegraphics[width=0.15\textwidth]{Figures/vis_realworld_sup/NPE_input.jpg} \hspace{-4mm} &
% \includegraphics[width=0.12\textwidth]{./Figures/vis_realworld/DICM_SNRNet.png} \hspace{-4mm} &
\includegraphics[width=0.15\textwidth]{Figures/vis_realworld_sup/NPE_Sparse.png} \hspace{-4mm} &
\includegraphics[width=0.15\textwidth]{Figures/vis_realworld_sup/NPE_Hint.png} \hspace{-4mm} 
\\
 Input \hspace{-4mm} &
% (b) SNRNet \hspace{-4mm} &
% 22.08 dB/LG-ShadowNet~\cite{liu2021lgshadow} \hspace{-4mm} &
 Sparse~\cite{yang2021sparse} \hspace{-4mm} &
 HINT \hspace{-4mm} 
\\
\includegraphics[width=0.15\textwidth,height=2cm]{Figures/vis_realworld_sup/VV_input.png} \hspace{-4mm} &
% \includegraphics[width=0.12\textwidth]{./Figures/vis_realworld/DICM_SNRNet.png} \hspace{-4mm} &
\includegraphics[width=0.15\textwidth,height=2cm]{Figures/vis_realworld_sup/VV_SNR-Net.png} \hspace{-4mm} &
\includegraphics[width=0.15\textwidth,height=2cm]{Figures/vis_realworld_sup/VV_Hint.png} \hspace{-4mm} 
\\
 Input \hspace{-4mm} &
% (b) SNRNet \hspace{-4mm} &
% 22.08 dB/LG-ShadowNet~\cite{liu2021lgshadow} \hspace{-4mm} &
 Sparse~\cite{yang2021sparse} \hspace{-4mm} &
 HINT \hspace{-4mm} 
\\
\end{tabular}
\end{adjustbox}
\end{tabular}
% \vspace{-2mm}
\caption{Visualizations on the real-world benchmarks, including NPE~\cite{wang2013naturalness}, DICM\cite{lee2013contrast}, VV~\cite{vonikakis2018evaluation}, and MEF~\cite{ma2015perceptual}. 
%
% For the input images, whether it's the building, the scene with birds, or the portrait, HINT avoids the issues of insufficient detail and inaccurate color representation. In contrast to SNRNet~\cite{xu2022snr} and Sparse~\cite{yang2021sparse}, HINT enhances the overall clarity, making architectural details of the building sharper, the feathers of the birds more distinct, and the facial features of the person clearer. Meanwhile, HINT also ensures more natural - looking colors across different scenes.
}
% \vspace{-2mm}
\label{pic:vis_realworld_supply}
\end{figure}


% \clearpage
%LOLv2_Fig
\begin{figure*}[htp!]
\footnotesize
\centering
\begin{tabular}{ccc}
\hspace{-0.42cm}
\begin{adjustbox}{valign=t}
\begin{tabular}{cccccccc}
\includegraphics[width=0.12\textwidth]{Figures/vis_LOLv2_syn/syn_input_1.png} \hspace{-4mm} &
\includegraphics[width=0.12\textwidth]{Figures/vis_LOLv2_syn/syn_gt_1.png} \hspace{-4mm} &
\includegraphics[width=0.12\textwidth]{Figures/vis_LOLv2_syn/syn_KinD_1.png} \hspace{-4mm} &
\includegraphics[width=0.12\textwidth]{Figures/vis_LOLv2_syn/syn_RUAS_1.png} \hspace{-4mm} &
\includegraphics[width=0.12\textwidth]{Figures/vis_LOLv2_syn/syn_MIRNet_1.png} \hspace{-4mm} &
\includegraphics[width=0.12\textwidth]{Figures/vis_LOLv2_syn/syn_Sparse_1.png} \hspace{-4mm} &
\includegraphics[width=0.12\textwidth]{Figures/vis_LOLv2_syn/syn_Restormer_1.png} \hspace{-4mm} &
\includegraphics[width=0.12\textwidth]{Figures/vis_LOLv2_syn/syn_hint_1.png} \hspace{-4mm} 
\\
\includegraphics[width=0.12\textwidth]{Figures/vis_LOLv2_real/input1.png} \hspace{-4mm} &
\includegraphics[width=0.12\textwidth]{Figures/vis_LOLv2_real/gt1.png} \hspace{-4mm} &
\includegraphics[width=0.12\textwidth]{Figures/vis_LOLv2_real/Kind1.png} \hspace{-4mm} &
\includegraphics[width=0.12\textwidth]{Figures/vis_LOLv2_real/RUAS1.png} \hspace{-4mm} &
\includegraphics[width=0.12\textwidth]{Figures/vis_LOLv2_real/MIRNet1.png} \hspace{-4mm} &
\includegraphics[width=0.12\textwidth]{Figures/vis_LOLv2_real/Sparse1.png} \hspace{-4mm} &
\includegraphics[width=0.12\textwidth]{Figures/vis_LOLv2_real/Restormer1.png} \hspace{-4mm} &
\includegraphics[width=0.12\textwidth]{Figures/vis_LOLv2_real/hint1.png} \hspace{-4mm} 
\\
(a) Input \hspace{-4mm} &
(b) Reference \hspace{-4mm} &
% 22.08 dB/LG-ShadowNet~\cite{liu2021lgshadow} \hspace{-4mm} &
(c) KinD~\cite{zhang2019kindling} \hspace{-4mm} &
(d) RUAS~\cite{liu2021retinex} \hspace{-4mm} &
(e) MIRNet~\cite{zamir2020learning} \hspace{-4mm} &
(f) {Sparse}~\cite{yang2021sparse} \hspace{-4mm} &
(g) {Restormer}~\cite{zamir2022restormer} \hspace{-4mm} &
(h) {HINT} (Ours) \hspace{-4mm} 

\\
\end{tabular}
\end{adjustbox}
\end{tabular}
\vspace{-2mm}
\caption{Qualitative results on LOL-v2~\cite{yang2021sparse} for low-light enhancement. 
%
The top case is from the synthetic subset, whereas the bottom one is from the real subset. 
%
% Compared to other techniques, HINT produces well-illuminated images, maintaining accurate colors and clear details. In contrast, other methods typically cause color inaccuracies or result in a loss of sharpness during the enhancement process.
}
% \vspace{-2mm}
\label{pic:enhancement_lolv2_supply}
\end{figure*}

%Snow_Fig
\begin{figure*}[htp!]
% \scriptsize
\footnotesize
\centering
\begin{tabular}{ccc}
\hspace{-0.42cm}
\begin{adjustbox}{valign=t}
\begin{tabular}{ccccccc}
\includegraphics[width=0.135\textwidth]{./Figures/vis_snow/input2.png} \hspace{-4mm} &
\includegraphics[width=0.135\textwidth]{./Figures/vis_snow/gt2.png} \hspace{-4mm} &
\includegraphics[width=0.135\textwidth]{./Figures/vis_snow/HDCW2.png} \hspace{-4mm} &
\includegraphics[width=0.135\textwidth]{./Figures/vis_snow/JSTASR2.png} \hspace{-4mm} &
\includegraphics[width=0.135\textwidth]{./Figures/vis_snow/Uformer2.png} \hspace{-4mm} &
\includegraphics[width=0.135\textwidth]{./Figures/vis_snow/AST2.png} \hspace{-4mm} &
\includegraphics[width=0.135\textwidth]{./Figures/vis_snow/hint2.png} \hspace{-4mm} 
\\
(a) Input \hspace{-4mm} &
(b) Reference \hspace{-4mm} &
% 22.08 dB/LG-ShadowNet~\cite{liu2021lgshadow} \hspace{-4mm} &
(c) HDCW~\cite{Chen_2021_ICCV} \hspace{-4mm} &
(d) JSTASR~\cite{chen2020jstasr} \hspace{-4mm} &
(e) Uformer~\cite{wang2022uformer} \hspace{-4mm} &
(f) {AST}~\cite{zhou2024AST} \hspace{-4mm} &
(g) {HINT} (Ours) \hspace{-4mm} 
\\
\end{tabular}
\end{adjustbox}
\end{tabular}
\vspace{-2mm}
\caption{Qualitative results on Snow100K~\cite{liu2018desnownet} for snow removal. 
}
\vspace{-2mm}
\label{pic:snow_supply}
\end{figure*}


%Denoise_Fig
\begin{figure*}
% \footnotesize
\scriptsize
\centering
\begin{tabular}{ccc}
% % one row
\begin{adjustbox}{valign=t}
\begin{tabular}{ccccc}
\hspace{-3mm}\includegraphics[width=0.19\textwidth]{Figures/noise_fig/input_15.png}  &
\hspace{-3mm}\includegraphics[width=0.19\textwidth]{Figures/noise_fig/gt_15.png}   &
\hspace{-3mm}\includegraphics[width=0.19\textwidth]{Figures/noise_fig/airnet_15.png}  &
\hspace{-3mm}\includegraphics[width=0.19\textwidth]{Figures/noise_fig/promptir_15.png}  &
\hspace{-3mm}\includegraphics[width=0.19\textwidth]{Figures/noise_fig/hint_15.png}  
\\
\hspace{-3mm}\includegraphics[width=0.19\textwidth]{Figures/noise_fig/input_25.png}  &
\hspace{-3mm}\includegraphics[width=0.19\textwidth]{Figures/noise_fig/gt_25.png}   &
\hspace{-3mm}\includegraphics[width=0.19\textwidth]{Figures/noise_fig/airnet_25.png}  &
\hspace{-3mm}\includegraphics[width=0.19\textwidth]{Figures/noise_fig/promptir_25.png}  &
\hspace{-3mm}\includegraphics[width=0.19\textwidth]{Figures/noise_fig/hint_25.png}   
\\
\hspace{-3mm}\includegraphics[width=0.19\textwidth]{Figures/noise_fig/input_50.png}  &
\hspace{-3mm}\includegraphics[width=0.19\textwidth]{Figures/noise_fig/gt_50.png}   &
\hspace{-3mm}\includegraphics[width=0.19\textwidth]{Figures/noise_fig/airnet_50.png}  &
\hspace{-3mm}\includegraphics[width=0.19\textwidth]{Figures/noise_fig/promptir_50.png}  &
\hspace{-3mm}\includegraphics[width=0.19\textwidth]{Figures/noise_fig/hint_50.png}  
\\
\hspace{-3mm}(a)   &
\hspace{-3mm}(b)   &   
\hspace{-3mm}(c)   &
\hspace{-3mm}(d)   &
\hspace{-3mm}(e) 
\\
\hspace{-3mm} Input &
\hspace{-3mm} Reference  &   
\hspace{-3mm} AirNet\cite{li2022all}  &
\hspace{-3mm} promptir \cite{potlapalli2024promptir}  &
\hspace{-3mm} HINT
\\
\end{tabular}
\end{adjustbox}
\end{tabular}
\vspace{-2mm}
\caption{Qualitative results on BSD68 \cite{martin2001database} benchmark for denoising.From the first row to the third row, respectively: noise levels of 15, 25, 50 denoising effect comparison
%
}
\vspace{-4mm}
\label{pic:vis_dehnoising_supply_BSD68}
\end{figure*}




\clearpage 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%notation table%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{0.5cm}
\onecolumn
\begin{longtable}[htbp]{c p{10.1cm} p{3cm}}
% \renewcommand{\arraystretch}{1.3}
% \centering
\captionsetup{margin=3pt}
\caption{Summary of the main notations in the manuscript as well as the corresponding descriptions. P, L, Func. and Tab. represent Page, Line, Function and Table, respectively. }\label{notation}\\
\hline
% \multicolumn{2}{c }{Begin of Table}\\
% \hline
\textbf{Notation} & \textbf{Description} & \textbf{Position}\\
\hline
\endfirsthead
\hline
\multicolumn{2}{c}{Continuation of Table \ref{notation}}\\
\hline
% \textbf{Notation} & \textbf{Description} & \textbf{Location}\\
\textbf{Notation} & \textbf{Description} & \textbf{Position}\\
\hline
\endhead
\hline
\multicolumn{3}{c}{Continued on next page}\\
\endfoot
\hline
\endlastfoot            
            $\mathbf{I}$ & the degraded image & P3, L172\\
            $H, W, C$ & the image height, width and the number of channels & P3, L174 \\
            $\mathbf{F}_s$ & the shallow feature & P3, L173 \\
            $N_1$ & the level of encoder-decoder restoration pipeline & P3, L176 \\
            $\mathbf{F}_d$ & the deep feature & P3, L177 \\
            $N_2$ & the number of basic blocks & P3, L178\\
            $\mathbf{R}$ & the residual image & P3, L191\\
            $\mathbf{\hat{I}}$ & the restored image  &P3, L193\\
            $\mathbf{X}$ & the normalized input tensor & P4, L204\\
            $\mathbf{Q}$, $\mathbf{K}$, $\mathbf{V}$ & the projection matrices in MHA mechanism & P4, Func. (1)\\
            $\mathbf{W}_Q,~\mathbf{W}_K,~\mathbf{W}_V $ & the linear projection matrices of the queries, keys, and values &P4, Func. (1)\\
            $d_k$, $d_v$ & the dimension of key and value & P4, L209\\
            $h$ & the number of heads in the standard MHA mechanism & P4, L214 \\
            $d_k/h$ & the dimension of subspace in MHA & P4,L216\\
            $\mathbf{W}_p $ & the output projection matrice for feature aggregation captured by heads & P4, Func. (2)\\
            % $\mathrm{H_{i}}$ & ? & P4, Func. (2)\\
            % \text{MultiHead(X)} & ? & P4, Func. (2)\\
            % \text{Concat} & the concatenation operation & P4, Func. (2)\\
            % \text{Attention} & ? & P4, Func. (2)\\
            $d_{out}$ & the dimension of the output projection matrice & P4, L220\\
            $C_i$ & the dimension of the i-th subspace in HMHA & P4, L267\\
            $\mathbf{F_{intra}}$ & the tensor of IntraCache & P4, L243\\
            $\mathbf{F_{out}}$ & the output tensor of MHA &P4, L244\\
            $\mathbf{F^{s}_{intra}}$ & the sum of $\mathbf{F_{intra}}$ and $\mathbf{F_{out}}$ & P4, L245\\
            $\mathbf{F_{gated}}$ & the result of gating mechanism & P4, Func. (3)\\
            $\odot$ & the element-wise product & P4, Func. (3)\\
            ${\rm Conv}(\cdot)$ & the convolution operation & P4, Func. (3)\\
            ${\rm GELU}(\cdot)$ & the GELU activation function & P4, Func. (3)\\
            $\mathbf{F^{o}_{Intra}}$ & the output feature after modulation process & P4, Func. (4)\\
            $\rm{Conv_{up}(\cdot)}$,$\rm{Conv_{down}(\cdot)}$ & the convolution operations that project the channel dimension into higher/lower levels & P4, Func. (4)\\
            % $\mathbf{Q^{i}},~\mathbf{K^{i}}$ & the i-th query and key projection matrices ? & P4, Func. (5)\\
            $\mathbf{F^{i}}$ & the sum of $\mathbf{Q^{i}}$ and $\mathbf{K^{i}}$ & P4, Func. (5)\\
            $\mathbf{F_{intra}}$ &  the Intra Query-Key Cache in each layer & P4, Func. (5)\\
            $\mathbf{F_{inter}}$ & the tensor of the InterCache & P4, L266\\
            $\mathbf{F_{att}}$ & dot-product attention of query and key & P4, L267\\
            $\mathbf{\hat{F}_{inter}}$ &  the resized feature map & P4, L268\\
            $\mathbf{F^{s}_{inter}}$ & the sum of $\mathbf{F_{att}}$ and $\mathbf{\hat{F}_{inter}}$ & P4, L271\\
            $\mathbf{F_{shift}}$ & shift component & P4, Func. (6)\\
            $\mathbf{F_{scale}}$ & scale component & P4, Func. (6)\\
            $\mathbf{W_{scale}}$,$\mathbf{W_{shift}}$ & the projection matrices that learned for scale $\mathbf{F_{scale}}$ and shift $\mathbf{F_{shift}}$ components & P4, Func. (6)\\
            $\mathbf{F_{m}}$ & the modified feature map & P4, Func. (6)\\
            $\mathbf{F^{o}_{inter}}$ & the output feature after inter modulation process & P5, Func. (7)\\
            $\mathbf{F}^{l}_{\mathbf{inter}}$ & the cache of the current layer & P5, Func. (8)\\
            $\rm{R}(\cdot)$ & the function that resizes the feature map of each head to the same shape & P5, Func. (8)\\
            $C_i/C$ & the assigned weight of each feature & P5, Func. (8)\\
            $\alpha$ & the weight that controls the degree of information flows within inter-layer cache & P5, Func. (9)\\
            
\end{longtable}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\twocolumn



